Truncated Wigner function theory of coherent Ising machines based on degenerate optical parametric oscillator network

We present the quantum theory of coherent Ising machines based on networks of degenerate optical parametric oscillators (DOPOs). In a simple model consisting of two coupled DOPOs, both positive-$P$ representation and truncated Wigner representation predict quantum correlation and inseparability between the two DOPOs in spite of the open-dissipative nature of the system. Here, we apply the truncated Wigner representation method to coherent Ising machines with thermal, vacuum, and squeezed reservoir fields. We find that the probability of finding the ground state of a one-dimensional Ising model increases substantially as a result of reducing excess thermal noise and squeezing the incident vacuum fluctuation on the out-coupling port.

==> pgf.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


\edef\pgfatcode{\the\catcode`\@}
\catcode`\@=11


\input pgfrcs.tex
\ProvidesPackageRCS $Header: /cvsroot/pgf/pgf/plain/pgf/basiclayer/pgf.tex,v 1.10 2008/01/15 17:17:22 tantau Exp $

\input pgfcore.tex

\usepgfmodule{shapes,plot}

%\input pgfbasesnakes.tex
%\input pgfbasedecorations.tex
%\input pgfbasematrix.tex

\catcode`\@=\pgfatcode

\endinput


==> pgffor.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\edef\pgfforatcode{\the\catcode`\@}
\catcode`\@=11

\input pgfrcs.tex
\input pgfkeys.code.tex
\input pgffor.code.tex

\catcode`\@=\pgfforatcode

\endinput

